Towards a Rigorous Evaluation of Time-series Anomaly Detection

In recent years, proposed studies on time-series anomaly detection (TAD) report high F1 scores on benchmark TAD datasets, giving the impression of clear improvements in TAD. However, most studies apply a peculiar evaluation protocol called point adjustment (PA) before scoring. In this paper, we theoretically and experimentally reveal that the PA protocol has a great possibility of overestimating the detection performance; that is, even a random anomaly score can easily turn into a state-of-the-art TAD method. Therefore, the comparison of TAD methods after applying the PA protocol can lead to misguided rankings. Furthermore, we question the potential of existing TAD methods by showing that an untrained model obtains comparable detection performance to the existing methods even when PA is forbidden. Based on our findings, we propose a new baseline and an evaluation protocol. We expect that our study will help a rigorous evaluation of TAD and lead to further improvement in future researches.

==> 00.Dependency.tex <==
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{lipsum}
\usepackage{threeparttable}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bm}
\usepackage{kotex}
\usepackage{color}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage{pifont}
\usepackage{cite}
\usepackage{tabularx}
\usepackage{float}
\usepackage{graphicx}
\usepackage{capt-of}
\newcommand{\xmark}{\ding{55}}
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}
\usepackage{amsthm}
\usepackage{arydshln}
\usepackage{adjustbox}
\newtheorem{prop}{Proposition}
\usepackage{mathtools}
\newcommand{\etal}{\textit{et al}.~}
\newcommand{\attr}{$\bm{\mathcal{I}}_{\Delta}(\bm{w}_{t,\tau})$}
\newcommand{\window}{\bm{w}_{t}}
\newcommand{\pa}{\texttt{PA}}
\newcommand{\anoscore}{\mathcal{A}\left(\window\right)}
\newcommand{\pak}{\texttt{PA\%K}}
\newcommand{\fpa}{$\texttt{F1}_\texttt{PA}$}
\newcommand{\fwpa}{$\texttt{F1}$}
\newcommand{\fnpa}{F1 score before \pa }
\newcommand{\red}[1]{\textcolor{black}{#1}}
\newcommand{\fswpa}{$\texttt{F1}_\texttt{PA}$}
\newcommand{\ing}{\textcolor{red}{ing}}
\newcommand{\todo}{\textcolor{green}{todo}}
\newcommand{\rep}[1]{#1$^{\dagger}$}
\usepackage{relsize,amsfonts}
\newcommand\bigexists{%
  \mathop{\lower0.75ex\hbox{\ensuremath{%
    {{\mathlarger{\mathlarger{\exists}}}}}}}%
  \limits}
\newcommand{\fpak}{$\texttt{F1}_\pak$}
\newcommand{\aupak}{$\texttt{AUPR}_\pak$}
\newcommand{\hi}{(\scalebox{0.8}{\textcolor{green}{$\uparrow$}})}
\newcommand{\lo}{(\scalebox{0.8}{\textcolor{red}{$\downarrow$}})}

% \newcommand{\pa}{\textbf{\texttt{PA}}~}
% \newcommand{\fpa}{F1 score after \pa }
% 
\usepackage[symbol]{footmisc}
\renewcommand{\thefootnote}{\fnsymbol{footnote}}


==> Table/dataset_statistics.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{l|rrr}
\toprule
     Dataset &Train  &Test (anomaly\%) & $N$ \\
\midrule
\textbf{SWaT} & 495,000                 &449,919    (12.33\%)                  & 51   \\
\textbf{WADI} & 784,537                  & 172,801 (5.77\%)                    & 123  \\
\textbf{SMD}  & 25,300                   & 25,300 (4.21\%)                     & 38   \\
\textbf{MSL} &58,317 &73,729 (10.5\%) &55 \\
\textbf{SMAP} &135,183 &427,617 (12.8\%) &25 \\
% \textbf{GHL}  & 1,535,118                  & 204,615 (0.39\%)                     & 6 &10 &5 &10   \\
\bottomrule
\end{tabular}
\caption{Statistics of benchmark TAD datasets. $N$ denotes the dimension of input features.}
\label{table:dataset_statistics}
\end{table}

==> Table/random_comparison.tex <==
\begin{table*}[t!]
% \centering 
% \resizebox{2.1\columnwidth}{!}{
\begin{adjustbox}{width=2.1\columnwidth,center}
\begin{tabular}{ccccccccccc}
\toprule
       & \multicolumn{2}{c}{\textbf{SWaT}} & \multicolumn{2}{c}{\textbf{WADI}} & \multicolumn{2}{c}{\textbf{MSL}} & \multicolumn{2}{c}{\textbf{SMAP}} & \multicolumn{2}{c}{\textbf{SMD}} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
       & \fpa      & \fwpa      & \fpa      & \fwpa     & \fpa      & \fwpa    & \fpa      & \fwpa      & \fpa      & \fwpa     \\
\midrule
USAD &0.846 \lo &\underline{0.791} \hi &0.429 \lo&0.232 \lo&\underline{0.927} \lo&0.211$^{\dagger}$ \lo &\underline{0.818} \lo&0.228$^{\dagger}$ \lo &\underline{0.938}\hi &0.426$^{\dagger}$ \lo\\
% $\text{USAD}^{\dagger}$ &0.8572 &0.7502 & & &0.7493 & &0.6389 &0.2268 &0.9382 &0.426  \\\hdashline
DAGMM &0.853 \lo &0.550 \lo&0.209 \lo&0.121 \lo&0.701 \lo&\rep{0.199} \lo &0.712 \lo&\rep{\textbf{0.333}} \hi &0.723 \lo  &\rep{0.238} \lo\\
LSTM-VAE &0.805 \lo &0.775 \lo&0.380 \lo&0.227 \lo&0.678 \lo&\rep{0.212} \lo &0.756 \lo&\rep{0.235} \hi &0.808 \hi &\rep{0.435} \lo \\
OmniAnomaly &0.866 \lo&0.782 \lo&0.417 \lo&0.223 \lo&0.899 \lo&\rep{0.207} \lo &0.805 \lo&\rep{0.227} \lo &\textbf{0.944} \hi &0.474$^{\dagger}$ \lo\\
MSCRED &0.868 \lo&\rep{0.662} \lo&0.346 \lo&\rep{0.087} \lo&0.775 \lo&\rep{0.199} \lo &\rep{0.942} \lo&\rep{0.232} \hi&  \rep{0.389} \lo&\rep{0.097} \lo\\ 
% $\text{MSCRED}^{\dagger}$ & &\textcolor{blue}{0.608} & &\textcolor{blue}{0.2380} & &\textcolor{blue}{0.1995} &\textcolor{blue}{0.4328} &\textcolor{blue}{0.1367} &  \textcolor{red}{0.2368}&\textcolor{red}{0.0624} \\ \hdashline
% MSCRED (WADI down-sampled): 0.289 (0.493)
%\textcolor{blue}{0.4526}&\textcolor{blue}{0.2065} \\ MSCRED (SMD 한번에)
% MAD-GAN &0.8690 &0.77 &0.373 &\ing &0.8747 &\ing &\ing &\ing &\ing  &\ing \\
THOC &0.880 \lo&0.612$^{\dagger}$ \lo&0.506 \lo&\rep{0.130} \lo&0.891 \lo &0.190$^{\dagger}$ \lo &0.781$^{\dagger}$ \lo&0.240$^{\dagger}$ \hi& 0.541$^{\dagger}$ \lo & \rep{0.168} \lo  \\ %\red{0.4766}&\red{0.1782}  \\ 따로할 때 더 성능이 안좋네요
% GTA &0.9134 & &0.8376 & &0.9110 & & & & &  \\
GDN &\underline{0.935} \lo&\textbf{0.81} \hi&\underline{0.855} \lo&\textbf{0.57} \hi &0.903 \lo&0.217$^{\dagger}$ \lo &\rep{0.708} \lo &\underline{0.252}$^{\dagger}$ \hi &\rep{0.716} \lo & \textbf{0.529}$^{\dagger}$ \hi\\
% SOTA &0.8460 &0.7917 &0.6198 &0.2328 &0.9109 &N/A &0.8186 &N/A &\textbf{0.9441} &N/A \\
\midrule
\textbf{Case 1} &\textbf{0.969} &0.216 &\textbf{0.965} &0.109 &\textbf{0.931} &0.190 &\textbf{0.961} &0.227 &0.804 &0.080 \\
\textbf{Case 2}   &0.873 &0.781 &0.694 &\underline{0.353} &0.812 & \underline{0.239} &0.675 &0.229 &0.896 &\underline{0.494} \\
\textbf{Case 3} &0.869 &0.789 &0.695 &0.331 &0.427 &\textbf{0.236} &0.699 &0.229 &0.893 &0.466  \\%msl window size 60
\bottomrule
\end{tabular}
% }
\end{adjustbox}
\caption{F1 score for various methods. $\dagger$ indicates the reproduced results. Bottom three rows represent the followings: \textbf{Case 1}. Random anomaly score, \textbf{Case 2}. Input itself as a anomaly score, \textbf{Case 3}. Anomaly score from a randomized model. Please refer to the manuscript for the detailed explanations. Bold and underlined cases indicate the best and the second best, respectively. \textcolor{green}{$\uparrow$} is marked in the following cases: (1) \fpa~is higher than \textbf{Case 1}, (2) \fwpa~is higher than \textbf{Case 2} or \textbf{3}.}
\label{table:random_comparsion}
\end{table*}




















% \begin{table*}[t!]
% \centering 
% \begin{tabular}{ccccccccccc}
% \toprule
%       & \multicolumn{2}{c}{\textbf{SWaT}} & \multicolumn{2}{c}{\textbf{WADI}} & \multicolumn{2}{c}{\textbf{MSL}} & \multicolumn{2}{c}{\textbf{SMAP}} & \multicolumn{2}{c}{\textbf{SMD}} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
%       & w/ \pa      & w/o \pa      & w/ \pa      & w/o \pa      & w/ \pa      & w/o \pa     & w/ \pa      & w/o \pa      & w/ \pa      & w/o \pa     \\
% \midrule
% USAD &0.846 \lo &\underline{0.791} \hi &0.4296 \lo&0.2328 \lo&\underline{0.9272} \lo&0.2112$^{\dagger}$ \lo &\underline{0.8186} \lo&0.2280$^{\dagger}$ \lo &\underline{0.9382}\hi &0.4265$^{\dagger}$ \lo\\
% % $\text{USAD}^{\dagger}$ &0.8572 &0.7502 & & &0.7493 & &0.6389 &0.2268 &0.9382 &0.426  \\\hdashline
% DAGMM &0.853 \lo &0.550 \lo&0.2094 \lo&0.1216\ \lo&0.7007 \lo&\rep{0.1987} \lo &0.7124 \lo&\rep{\textbf{0.3330}} \hi &0.7231 \lo  &\rep{0.2387} \lo\\
% LSTM-VAE &0.805 \lo &0.775 \lo&0.3799 \lo&0.2271 \lo&0.6780 \lo&\rep{0.2127} \lo &0.7555 \lo&\rep{0.2352} \hi &0.8083 \hi &\ing \\
% OmniAnomaly &0.866 \lo&0.782 \lo&0.4174 \lo&0.2296 \lo&0.8990 \lo&\rep{0.2074} \lo &0.8054 \lo&\rep{0.2272} \lo &\textbf{0.944} \hi &\underline{0.4745}$^{\dagger}$ \hi\\
% MSCRED &0.868 \lo&\rep{0.608} \lo&0.3458 \lo&\rep{0.0869} \lo&0.7745 \lo&\rep{0.1995} \lo &\rep{0.9423} \lo&\rep{0.2322} \hi&  \rep{0.3892} \lo&\rep{0.0968} \lo\\ 
% % $\text{MSCRED}^{\dagger}$ & &\textcolor{blue}{0.6087} & &\textcolor{blue}{0.0869} & &\textcolor{blue}{0.1995} &\textcolor{blue}{0.4328} &\textcolor{blue}{0.1367} &  \textcolor{red}{0.2368}&\textcolor{red}{0.0624} \\ \hdashline
% %\textcolor{blue}{0.4526}&\textcolor{blue}{0.2065} \\ 따로할 때 더 성능이 안좋네요
% % MAD-GAN &0.8690 &0.77 &0.373 &\ing &0.8747 &\ing &\ing &\ing &\ing  &\ing \\
% THOC &0.880 \lo&0.612$^{\dagger}$ \lo&0.5059 \lo&\rep{0.1296} \lo&0.8906 \lo &0.1903$^{\dagger}$ \lo &0.7812$^{\dagger}$ \lo&0.2397$^{\dagger}$ \hi& 0.5415$^{\dagger}$ \lo & \rep{0.1682} \lo  \\ %\red{0.4766}&\red{0.1782}  \\ 따로할 때 더 성능이 안좋네요
% % GTA &0.9134 & &0.8376 & &0.9110 & & & & &  \\
% GDN &\underline{0.935} \lo&\textbf{0.81} \hi&\underline{0.8552} \lo&\textbf{0.57} \hi &0.9033 \lo&\underline{0.2167}$^{\dagger}$ \lo &\rep{0.7083} \lo &\underline{0.2516}$^{\dagger}$ \hi &\rep{0.7163} \lo & \textbf{0.5290}$^{\dagger}$ \hi\\
% % SOTA &0.8460 &0.7917 &0.6198 &0.2328 &0.9109 &N/A &0.8186 &N/A &\textbf{0.9441} &N/A \\
% \midrule
% \textbf{Case 1} &\textbf{0.969} &0.2164 &\textbf{0.9645} &0.1093 &\textbf{0.9309} &0.1908 &\textbf{0.9606} &0.2268 &0.8036 &0.0801 \\
% \textbf{Case 2}   &0.873 &0.7868 &0.6937 &\underline{0.3385} &0.8121 & 0.2135 &0.6748 &0.2272 &0.8964 &0.4660 \\
% \textbf{Case 3} &0.869 &0.7889 &0.6954 &0.3307 &0.8833 &\textbf{0.2364} &0.6992 &0.2289 &0.8933 &0.4663  \\%msl window size 60
% \bottomrule
% \end{tabular}
% \caption{F1 score for various methods. $\dagger$ indicates the reproduced results. Bottom three rows represent the followings: \textbf{Case 1}. Random anomaly score, \textbf{Case 2}. Input itself as a anomaly score, \textbf{Case 3}. Anomaly score from a randomized model. Please refer to the manuscript for the detailed explanations. Bold and underlined cases indicate the best and the second best, respectively.}
% \label{table:random_comparsion}
% \end{table*}

